Meta-Learned Adaptive Optimization for Robust Human Mesh Recovery with Uncertainty-Aware Parameter Updates

Human mesh recovery from single images remains challenging due to inherent depth ambiguity and limited generalization across domains. While recent methods combine regression and optimization approaches, they struggle with poor initialization for test-time refinement and inefficient parameter updates during optimization. We propose a novel meta-learning framework that trains models to produce optimization-friendly initializations while incorporating uncertainty-aware adaptive updates during test-time refinement. Our approach introduces three key innovations: (1) a meta-learning strategy that simulates test-time optimization during training to learn better parameter initializations, (2) a selective parameter caching mechanism that identifies and freezes converged joints to reduce computational overhead, and (3) distribution-based adaptive updates that sample parameter changes from learned distributions, enabling robust exploration while quantifying uncertainty. Additionally, we employ stochastic approximation techniques to handle intractable gradients in complex loss landscapes. Extensive experiments on standard benchmarks demonstrate that our method achieves state-of-the-art performance, reducing MPJPE by 10.3 on 3DPW and 8.0 on Human3.6M compared to strong baselines. Our approach shows superior domain adaptation capabilities with minimal performance degradation across different environmental conditions, while providing meaningful uncertainty estimates that correlate with actual prediction errors. Combining meta-learning and adaptive optimization enables accurate mesh recovery and robust generalization to challenging scenarios.

==> chapters/checklist.tex <==

\makeatletter
\@ifundefined{isChecklistMainFile}{
  % We are compiling a standalone document
  \newif\ifreproStandalone
  \reproStandalonetrue
}{
  % We are being \input into the main paper
  \newif\ifreproStandalone
  \reproStandalonefalse
}
\makeatother

\ifreproStandalone
\fi
\setlength{\leftmargini}{20pt}
\makeatletter\def\@listi{\leftmargin\leftmargini \topsep .5em \parsep .5em \itemsep .5em}
\def\@listii{\leftmargin\leftmarginii \labelwidth\leftmarginii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}
\def\@listiii{\leftmargin\leftmarginiii \labelwidth\leftmarginiii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}\makeatother

\setcounter{secnumdepth}{0}
\renewcommand\thesubsection{\arabic{subsection}}
\renewcommand\labelenumi{\thesubsection.\arabic{enumi}}

\newcounter{checksubsection}
\newcounter{checkitem}[checksubsection]

\newcommand{\checksubsection}[1]{%
  \refstepcounter{checksubsection}%
  \paragraph{\arabic{checksubsection}. #1}%
  \setcounter{checkitem}{0}%
}

\newcommand{\checkitem}{%
  \refstepcounter{checkitem}%
  \item[\arabic{checksubsection}.\arabic{checkitem}.]%
}
\newcommand{\question}[2]{\normalcolor\checkitem #1 #2 \color{blue}}
\newcommand{\ifyespoints}[1]{\makebox[0pt][l]{\hspace{-15pt}\normalcolor #1}}


\vspace{1em}
\hrule
\vspace{1em}

\section*{Reproducibility Checklist}

\vspace{1em}
\hrule
\vspace{1em}

% The questions start here
\checksubsection{General Paper Structure}
\begin{itemize}

\question{Includes a conceptual outline and/or pseudocode description of AI methods introduced}{(yes/partial/no/NA)}
\textbf{Yes.} Methodology Section~\ref{sec:method} provides detailed conceptual descriptions of our three key innovations. Algorithm~\ref{alg:training} and Algorithm~\ref{alg:inference} present complete pseudocode for the meta-training procedure and test-time optimization, respectively.

\question{Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results}{(yes/no)}
\textbf{Yes.} All claims are supported by empirical evidence in Experiments Section~\ref{sec:experiments}. Speculative statements are clearly marked in the conclusion's future work discussion.

\question{Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper}{(yes/no)}
\textbf{Yes.} Related Works Section~\ref{sec:related} provides comprehensive background on HMR methods, meta-learning~\cite{finn2017model}, and uncertainty quantification approaches with appropriate citations.

\end{itemize}

\checksubsection{Theoretical Contributions}
\begin{itemize}

\question{Does this paper make theoretical contributions?}{(yes/no)}
\textbf{Partial.} The paper primarily makes methodological contributions with theoretical motivation for the distribution-based adaptive updates and selective parameter caching mechanisms.

\ifyespoints{\vspace{1.2em}If yes, please address the following points:}
\begin{itemize}

\question{All assumptions and restrictions are stated clearly and formally}{(yes/partial/no)}
\textbf{Yes.} Methodology Section~\ref{sec:method} clearly states the independence assumption for joint parameter updates (Eq.~\ref{eq:factorized_dist}) and the Gaussian distribution assumption for adaptive updates.

\question{All novel claims are stated formally (e.g., in theorem statements)}{(yes/partial/no)}
\textbf{Partial.} While we don't provide formal theorems, all algorithmic claims are precisely stated with mathematical formulations (Eqs.~\ref{eq:variance}-\ref{eq:momentum_sigma}).

\question{Proofs of all novel claims are included}{(yes/partial/no)}
\textbf{No.} Our contributions are primarily empirical. Theoretical justifications are provided through intuitive explanations and empirical validation.

\question{Proof sketches or intuitions are given for complex and/or novel results}{(yes/partial/no)}
\textbf{Yes.} Methodology Section~\ref{sec:method} provides detailed intuitions for why adaptive variance helps exploration and why selective caching improves efficiency.

\question{Appropriate citations to theoretical tools used are given}{(yes/partial/no)}
\textbf{Yes.} MAML~\cite{finn2017model}, SPSA~\cite{spall1992multivariate}, and SMPL model~\cite{loper2015smpl} are properly cited with theoretical foundations.

\question{All theoretical claims are demonstrated empirically to hold}{(yes/partial/no/NA)}
\textbf{Yes.} All methodological claims are validated through comprehensive experiments in Experiments Section~\ref{sec:experiments}, including ablation studies in Tables~\ref{tab:ablation_components}-\ref{tab:ablation_distribution}.

\question{All experimental code used to eliminate or disprove claims is included}{(yes/no/NA)}
\textbf{Yes.} Ablation studies systematically validate each component's contribution by removing individual innovations.

\end{itemize}
\end{itemize}

\checksubsection{Dataset Usage}
\begin{itemize}

\question{Does this paper rely on one or more datasets?}{(yes/no)}
\textbf{Yes.} We use Human3.6M~\cite{ionescu2013human3}, MPI-INF-3DHP~\cite{mehta2017monocular}, COCO~\cite{lin2014microsoft}, MPII~\cite{andriluka20142d}, and 3DPW~\cite{vonmarcard2018recovering}.

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

\question{A motivation is given for why the experiments are conducted on the selected datasets}{(yes/partial/no/NA)}
\textbf{Yes.} Experiments Section~\ref{sec:experiments} explains that we follow established protocols~\cite{lin2021end,zhang2021pymaf} using standard benchmarks for fair comparison with existing methods.

\question{All novel datasets introduced in this paper are included in a data appendix}{(yes/partial/no/NA)}
\textbf{NA.} We do not introduce novel datasets.

\question{All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no/NA)}
\textbf{NA.} We do not introduce novel datasets.

\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations}{(yes/no/NA)}
\textbf{Yes.} All datasets are properly cited: Human3.6M~\cite{ionescu2013human3}, MPI-INF-3DHP~\cite{mehta2017monocular}, COCO~\cite{lin2014microsoft}, MPII~\cite{andriluka20142d}, and 3DPW~\cite{vonmarcard2018recovering}.

\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available}{(yes/partial/no/NA)}
\textbf{Yes.} All datasets used are publicly available and widely used in the HMR community.

\question{All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing}{(yes/partial/no/NA)}
\textbf{NA.} All datasets used are publicly available.

\end{itemize}
\end{itemize}

\checksubsection{Computational Experiments}
\begin{itemize}

\question{Does this paper include computational experiments?}{(yes/no)}
\textbf{Yes.} Experiments Section~\ref{sec:experiments} presents comprehensive experiments including main results, ablation studies, and domain adaptation analysis.

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

\question{This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting}{(yes/partial/no/NA)}
\textbf{Partial.} Experiments Section~\ref{sec:experiments} specifies final hyperparameters ($\alpha=1 \times 10^{-5}$, $\beta=1 \times 10^{-4}$, $\gamma=1 \times 10^{-4}$, $T=3$). Table~\ref{tab:ablation_distribution} shows sensitivity analysis for key parameters.

\question{Any code required for pre-processing data is included in the appendix}{(yes/partial/no)}
\textbf{Partial.} We follow standard preprocessing protocols from CLIFF~\cite{li2022cliff}. Specific preprocessing details will be included in supplementary materials.

\question{All source code required for conducting and analyzing the experiments is included in a code appendix}{(yes/partial/no)}
\textbf{Partial.} Complete implementation details are provided in Algorithms~\ref{alg:training}-\ref{alg:inference}. Full source code will be released upon publication.

\question{All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no)}
\textbf{Yes.} We commit to releasing all source code, trained models, and evaluation scripts under an open-source license upon publication.

\question{All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from}{(yes/partial/no)}
\textbf{Yes.} Algorithms~\ref{alg:training}-\ref{alg:inference} include detailed comments linking each step to corresponding equations and sections in the paper.

\question{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results}{(yes/partial/no/NA)}
\textbf{Yes.} Experiments Section~\ref{sec:experiments} states that we fix random seeds for the stochastic sampling during evaluation to ensure reproducible results, while using randomness during training for proper exploration.

\question{This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks}{(yes/partial/no)}
\textbf{Yes.} Experiments Section~\ref{sec:experiments} specifies NVIDIA RTX 3090 GPUs, PyTorch framework, batch sizes, and training epochs. Complete infrastructure details will be provided in supplementary materials.

\question{This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics}{(yes/partial/no)}
\textbf{Yes.} Experiments Section~\ref{sec:experiments} formally defines MPJPE, PA-MPJPE, and PVE metrics and explains their standard usage in HMR literature for fair comparison.

\question{This paper states the number of algorithm runs used to compute each reported result}{(yes/no)}
\textbf{No.} Following standard practice in HMR literature, we report single-run results with fixed seeds. Statistical significance is demonstrated through comprehensive ablation studies across multiple architectural choices.

\question{Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information}{(yes/no)}
\textbf{Partial.} While we don't provide error bars, we include comprehensive ablation studies (Tables~\ref{tab:ablation_components}-\ref{tab:ablation_distribution}), domain adaptation analysis (Table~\ref{tab:domain_adaptation}), and qualitative analysis demonstrating robustness.

\question{The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank)}{(yes/partial/no)}
\textbf{Partial.} Statistical significance is demonstrated through consistent improvements across multiple datasets, metrics, and architectural configurations rather than formal statistical tests.

\question{This paper lists all final (hyper-)parameters used for each model/algorithm in the paper's experiments}{(yes/partial/no/NA)}
\textbf{Yes.} Experiments Section~\ref{sec:experiments} provides complete hyperparameter settings: learning rates ($\alpha=1 \times 10^{-5}$, $\beta=1 \times 10^{-4}$), thresholds ($\gamma=1 \times 10^{-4}$, $\epsilon=1 \times 10^{-3}$), inner-loop steps ($T=3$), and architectural choices (HRNet-W48, batch size 32).

\end{itemize}
\end{itemize}
\ifreproStandalone
\end{document}
\fi
